Speaker Adaptive Training using Model Agnostic Meta-Learning

Speaker adaptive training (SAT) of neural network acoustic models learns models in a way that makes them more suitable for adaptation to test conditions. Conventionally, model-based speaker adaptive training is performed by having a set of speaker dependent parameters that are jointly optimised with speaker independent parameters in order to remove speaker variation. However, this does not scale well if all neural network weights are to be adapted to the speaker. In this paper we formulate speaker adaptive training as a meta-learning task, in which an adaptation process using gradient descent is encoded directly into the training of the model. We compare our approach with test-only adaptation of a standard baseline model and a SAT-LHUC model with a learned speaker adaptation schedule and demonstrate that the meta-learning approach achieves comparable results.

==> tables/lr_all.tex <==
\begin{table}[t!]
\begin{center}

\setlength{\tabcolsep}{0.4em}
\begin{tabularx}{\columnwidth}{Xrrrrrr}
            & \multicolumn{3}{c}{{Baseline}} & \multicolumn{3}{c}{{MAML}} \\
            & {10s} & {30s} & {60s} & {10s} & {30s} & {60s} \\
\hline
tdnn1       & 0.2 & 0.1 & 0.1 & 0.1 &  0.0 &  0.1 \\
tdnn1.bn    & 0.9 & 0.6 & 0.4 & 1.3 &  1.3 &  0.8 \\
tdnn2       & 1.2 & 0.7 & 0.6 & 1.8 &  1.9 &  1.4 \\
tdnn2.bn    & 0.8 & 0.5 & 0.3 & 1.0 &  0.7 &  0.2 \\
tdnn3       & 1.2 & 0.7 & 0.6 & 1.7 &  1.5 &  0.9 \\
tdnn3.bn    & 0.6 & 0.5 & 0.3 & 0.7 &  0.3 &  0.1 \\
tdnn4       & 1.3 & 0.8 & 0.7 & 2.0 &  2.0 &  1.4 \\
tdnn4.bn    & 0.6 & 0.4 & 0.3 & 0.5 & -0.1 & -0.3 \\
tdnn5       & 1.3 & 0.9 & 0.9 & 2.3 &  2.3 &  2.0 \\
tdnn5.bn    & 0.6 & 0.5 & 0.5 & 0.6 &  0.4 &  0.5 \\
tdnn6       & 1.3 & 0.9 & 0.9 & 2.2 &  2.3 &  2.2 \\
tdnn6.bn    & 0.1 & 0.1 & 0.1 & 0.1 &  0.0 &  0.1 \\
output      & 0.0 & 0.0 & 0.0 & 0.0 & -0.1 &  0.0 \\
\end{tabularx}

\caption{Learned learning rates for supervised adaptation of ALL parameters with varying amounts of adaptation data. (tdnn* correspond to TDNN affine layers and tdnn*.bn correspond to subsequent batch normalisation layers.)}

\label{table:lr_all}
\end{center}
\end{table}

==> tables/lr_lhuc.tex <==
\begin{table}[t!]
\begin{center}

\setlength{\tabcolsep}{0.4em}
\begin{tabularx}{\columnwidth}{Xrrrrrrrrr}
    & \multicolumn{3}{c}{{Baseline}} & \multicolumn{3}{c}{{SAT-LHUC}}  & \multicolumn{3}{c}{{MAML}} \\
layer    & {10s} & {30s} & {60s} & {10s} & {30s} & {60s} & {10s} & {30s} & {60s} \\
\hline
lhuc1 & 3.1 & 1.2 & 1.1 & 3.4 & 1.2 & 1.1 & 3.3 & 2.7 & 1.8 \\
lhuc2 & 3.0 & 1.2 & 1.1 & 3.5 & 1.3 & 1.1 & 3.3 & 2.7 & 1.9 \\
lhuc3 & 3.1 & 1.2 & 1.1 & 3.0 & 1.2 & 1.2 & 3.3 & 2.7 & 1.9 \\
lhuc4 & 2.7 & 1.2 & 1.1 & 3.0 & 1.3 & 1.2 & 3.0 & 2.3 & 1.8 \\
lhuc5 & 2.3 & 1.2 & 1.1 & 2.5 & 1.2 & 1.1 & 2.6 & 2.4 & 1.9 \\
lhuc6 & 2.5 & 1.2 & 1.2 & 2.4 & 1.2 & 1.1 & 2.7 & 2.4 & 2.3 \\
\end{tabularx}

\caption{Learned learning rates for supervised adaptation of LHUC parameters with varying amounts of adaptation data.}

\label{table:lr_lhuc}
\end{center}
\end{table}

==> tables/order_all.tex <==
\begin{table}[t!]
\begin{center}
\caption{WER(\%) of the supervised speaker adaptation of ALL parameters of the baseline model and MAML models that use first order and second order derivatives during training.}

\begin{tabularx}{\columnwidth}{Xcccccc}
\toprule
                        & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{First Order} & \multicolumn{2}{c}{Second Order} \\
						&  dev & test &  dev & test &  dev & test  \\
\midrule
original				& 15.3 & 13.4 & 18.4 & 16.2 & - & - \\
10s 					& 14.7 & 12.6 & 15.2 & 13.1 & - & - \\
30s						& 14.4 & 12.1 & - & - & - & - \\
60s 					& 14.0 & 11.7 & - & - & - & - \\
\bottomrule
\end{tabularx}
\label{table:order_all}
\end{center}
\end{table}

==> tables/order_lhuc.tex <==
\begin{table}[t!]
\begin{center}
\caption{WER(\%) of the supervised speaker adaptation of LHUC parameters of the baseline model and MAML models that use first order and second order derivatives during training.}
\begin{tabularx}{\columnwidth}{Xcccccc}
\toprule
                        & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{First Order} & \multicolumn{2}{c}{Second Order} \\
						&  dev & test &  dev & test &  dev & test  \\
\midrule
original				& 15.3 & 13.4 & 18.1 & 15.4 & - & - \\
10s 					& 14.8 & 12.7 & 14.8 & 12.7 & - & - \\
30s						& 14.6 & 12.5 & - & - & - & - \\
60s 					& 14.3 & 12.1 & - & - & - & - \\
\bottomrule
\end{tabularx}
\label{table:order_lhuc}
\end{center}
\end{table}
